Gated Attentive-Autoencoder for Content-Aware Recommendation

The rapid growth of Internet services and mobile devices provides an excellent opportunity to satisfy the strong demand for the personalized item or product recommendation. However, with the tremendous increase of users and items, personalized recommender systems still face several challenging problems: (1) the hardness of exploiting sparse implicit feedback; (2) the difficulty of combining heterogeneous data. To cope with these challenges, we propose a gated attentive-autoencoder (GATE) model, which is capable of learning fused hidden representations of items' contents and binary ratings, through a neural gating structure. Based on the fused representations, our model exploits neighboring relations between items to help infer users' preferences. In particular, a word-level and a neighbor-level attention module are integrated with the autoencoder. The word-level attention learns the item hidden representations from items' word sequences, while favoring informative words by assigning larger attention weights. The neighbor-level attention learns the hidden representation of an item's neighborhood by considering its neighbors in a weighted manner. We extensively evaluate our model with several state-of-the-art methods and different validation metrics on four real-world datasets. The experimental results not only demonstrate the effectiveness of our model on top-N recommendation but also provide interpretable results attributed to the attention modules.

==> preliminaries.tex <==
\section{Methods}
In this section, we demonstrate the proposed methodology for the task of POI recommendations, which takes POI similarities, user preferences and geographical influence into account.


\subsection{Notation}
Suppose there are $ N $ users and $ M $ locations. We denote the set of all locations as $ L $. For convenience we will henceforth refer to $ u $ as user and $ l $ as location. The terms location and POI are used interchangeably in this paper. In addition, the sequence a user $ u $ checked-in is denoted as $  S_{u} $, and the set a user $ u $ checked-in is referred to $  L_{u} $. Following common symbolic notation, upper case bold letters denote matrices, lower case bold letters denote column vectors without any specification, and non-bold letters represent scalars.







